New angles on standard force fields: towards a general approach for treating atomic-level anisotropy

Nearly all standard force fields employ the 'sum-of-spheres' approximation, which models intermolecular interactions purely in terms of interatomic distances. Nonetheless, atoms in molecules can have significantly non-spherical shapes, leading to interatomic interaction energies with strong orientation dependencies. Neglecting this 'atomic-level anisotropy' can lead to significant errors in predicting interaction energies. Herein we propose a simple, transferable, and computationally-efficient model (MASTIFF) whereby atomic-level orientation dependence can be incorporated into ab initio intermolecular force fields. MASTIFF includes anisotropic exchange-repulsion, charge penetration, and dispersion effects, in conjunction with a standard treatment of anisotropic long-range (multipolar) electrostatics. To validate our approach, we benchmark MASTIFF against various sum-of-spheres models over a large library of intermolecular interactions between small organic molecules. MASTIFF achieves quantitative accuracy with respect to both high-level electronic structure theory and experiment, thus showing promise as a basis for 'next-generation' force field development.

==> literature_outline.tex <==
%auto-ignore
Classical molecular simulations have become a standard tool in
interpreting and predicting the chemistry of a wide host of systems ranging
from simple liquids to complex materials and biomolecules. Such simulations
always require, as input, a mathematical description of the
system's $3N$-dimensional potential energy surface (PES). In principle, the
PES for most chemical systems can accurately be determined 
from one of several high-level electronic structure methods;
\cite{CCSDT, some reviews on EST and AIMD}
nevertheless, these types of calculations are computationally-intractable for
studying both large systems and/or long timescales. Consequently, most
molecular simulation today is performed with the aid of force fields,
broadly defined as computationally-inexpensive, parameterized mathematical expressions that
approximate the exact PES.

Given the prevalence of force fields in molecular simulation, it becomes
necessary to inquire: how successful are these force fields in enabling accurate and/or predictive
molecular simulation? Unsurprisingly, the answer often depends on a variety of
factors, particularly the choice of functional form (that is, mathematical
expression), the parameterization method, and the nature(s) of the chemical
interactions of study. 
% TODO: Look up reviews that study force fields as a function of chemical
% interaction
(As a particularly poignant example of how functional form and parameter
choice effects the quality of the resultant force field, one need look no
further than the myriad water potentials, results of which have been
summarized in \cite{Cisneros2016a}.)



% Look up refs 7-- 10 from \cite{Kramer2014}
% Look up refs 26-28 from \cite{Bartocci2015}
% Look up refs (and check for follow-up work) 61-62 in \cite{Elking2010}

============================================
Previous work on anisotropic electrostatics:
============================================
Off-site point charges (representing lone pairs or otherwise):
    How to place them, applications to acetone, methanol, methylamine, etc: \cite{Harder2006}
    Using ELF to determine off-site locations: \cite{Chaudret2013}
    Systematic investigation of improvements w/ off-site charges: \cite{Dixon1997}
        Conclusion: adding off-sites improves results
    Off-sites for halogens: \cite{Rendine2011}
Multipoles, Gaussian or point-charge: 
    AMOEBA, organochlorines: \cite{Mu2014}
    AMOEBA, general: \cite{Ren2003,Shi2013}
    GEM, theory: \cite{Cisneros2006}
    GEM, theory pt. 2: \cite{Elking2010}
    DMA, review: \cite{Stone2007}, \cite{Demerdash2014}
    SIBFA: \cite{Chaudret2014a}
    Example in water (SCME): \cite{Wikfeldt2013}
    mDC DFTB2 model (QM/MM work): \cite{Giese2013}
Importance of charge anisotropy for different functional groups
    Systematic overview of different functional groups: \cite{Kramer2014}
    In halogens (CX4, X=Cl, F) : \cite{Bartocci2015}
    Sigma-hole bonding: \cite{Politzer2008}

============================================
Previous work on anisotropic polarizabilities:
============================================
Anisotropic drude oscillators \cite{Harder2006}
Discussion of base stacking: \cite{Sponer2013}
    Suggests that isotropic atom model might overestimate strength of base
    stacking, leading to overstabilization of stacked arrangements in MD
    simulations
Off-site polarizabilities in SIBFA: \cite{Piquemal2007}

============================================
Previous work on anisotropic overlap effects:
============================================
Direct computation of (anisotropic) overlap integrals
    GEM model for water: \cite{Duke2014a}
    GEM, theory: \cite{Cisneros2006}
    GEM, theory pt. 2: \cite{Elking2010}
    SIBFA + GEM, application paper: \cite{Chaudret2014a}
    SCDS, theory: \cite{Gavezzotti2003}
        (model uses numerical integration, gets (with few parameters) results
         very close to SAPT for a number of organic systems)
Anisotropic Stone functional form:
    Shape functions, review: \cite{Stone2007}
Importance:
    In halogens (CX4, X=Cl, F) : \cite{Bartocci2015}


============================================
Previous work on anisotropic VdW radii:
============================================
Discussion of 'anisotropy of vdW radii': \cite{Hagler2015} and refs therein
Anisotropic VdW Radii, discussion from CSD
    Interactions between halogens and O,N; also IMPT calculations: \cite{Lommerse1996}
    Original Bondi Paper, assigned vdw radii and noticed that not all radii
        are isotropic: \cite{Bondi1964}
    Extension of Bondi's work, also notices anisotropy: \cite{Nyburg1985}
    More anisotropy: \cite{Batsanov2001}
    Anisotropic vdW radii in halogen bonding: \cite{Auffinger2004}
    'Flattening Factors' for VdW Anisotropy: \cite{Eramian2013}
Anisotropy, well-depth, experimental: \cite{Pack1978}
Anisotropic VdW Radii, discussion from electronic structure theory
    Natural steric analysis: \cite{Badenhoop1997a}
    CCSD(T), SAPT on homonuclear diatomics interacting with themselves, ions, water, and benzene: \cite{Kim2014b}
Gay-Berne potential (anisotropic LJ): \cite{Gay1981}


============================================
Previous work on anisotropic dispersion:
============================================
Generation of anisotropic dispersion coefficients, review: \cite{Stone2007}
Importance of dispersion anisotropy:
    in MM force fields: \cite{Zgarbova2010}
    in describing base stacking: \cite{Sponer2013}
QM description of pi systems: \cite{Krishtal2011}


============================================
Previous work on halogens:
============================================
AMOEBA, multipoles for organochlorine compounds: \cite{Mu2014}


============================================
Previous work on pi-stacking:
============================================
Difficulty in developing benzene models for standard force fields:
\cite{Sherrill2009}
    (Note: no discussion of anisotropy. Main complaint here is lack of charge
        penetration)


============================================
History of work in Sally's group, Anthony's group, etc.
============================================
First anisotropic potential for the repulsive wall (cyanuric chloride): \cite{Mitchell2001}
Review of anisotropic functional forms: \cite{Price2000}
Modeling crystals wtih multipoles and polarizability: \cite{Price2010a}
    No repulsion anisotropy here
Anisotropic Atom-Atom Potentials: \cite{Stone1988}
    "We shall argue that there is
    theoretical and experimental evidence to show that the molecular
    anisotropy cannot be represented adequately in terms of this sort
    of superposition of spherical atoms, and we shall show how to
    introduce anisotropy directly into the site-site interaction itself,
    using the same orientation-dependent functions that are required
    to describe the long-range forces."
Modeling PAHs with anisotropic repulsion: \cite{Totton2010}
ASP-W potential: \cite{Torheyden2006}
    Gaussian overlaps for electrostatic charge penetration
    Stone-form exchange
    Higher-order polarizabilities
    Multipole expansion dispersion




Goal: add anisotropy (higher-order moments) to improve description of both the
long-range and overlap regions.

Split into two categories: long-range (1/R)^n distance dependence, and
short-range (where overlap effects matter, and which decay exponentially)

What does our work add that previous work hasn't accomplished?
-- Add anisotropy to an 'ideal' (well, at least better than previous work)
isotropic potential
-- Address the general applicability of anisotropy for a diverse test set
-- Concretely address the transferability question
-- Provide an overall workflow for significantly improved anisotropic
potentials


